Copy Suppression: Comprehensively Understanding an Attention Head

We present a single attention head in GPT-2 Small that has one main role across the entire training distribution. If components in earlier layers predict a certain token, and this token appears earlier in the context, the head suppresses it: we call this copy suppression. Attention Head 10.7 (L10H7) suppresses naive copying behavior which improves overall model calibration. This explains why multiple prior works studying certain narrow tasks found negative heads that systematically favored the wrong answer. We uncover the mechanism that the Negative Heads use for copy suppression with weights-based evidence and are able to explain 76.9% of the impact of L10H7 in GPT-2 Small. To the best of our knowledge, this is the most comprehensive description of the complete role of a component in a language model to date. One major effect of copy suppression is its role in self-repair. Self-repair refers to how ablating crucial model components results in downstream neural network parts compensating for this ablation. Copy suppression leads to self-repair: if an initial overconfident copier is ablated, then there is nothing to suppress. We show that self-repair is implemented by several mechanisms, one of which is copy suppression, which explains 39% of the behavior in a narrow task. Interactive visualisations of the copy suppression phenomena may be seen at our web app https://copy-suppression.streamlit.app/

==> sections/archived/old_cspa_ablation_with_semantic_similarity.tex <==
\section{How Negative Heads Copy Suppress}
\label{sec:how_negative_heads_copy_suppress}

In this section, we explain mechanistically what Negative Heads such as 10.7 do on the general distribution.

Our mechanism for copy suppression explains X\% of 10.7’s contribution to reducing loss (Section 3.3). To reach this conclusion, we first describe a concrete mechanism for how head 10.7 works.

\begin{enumerate}
    \item In \Cref{subsec:ov_circuit}, we show that the head suppresses the prediction of any token which it attends to.
    \item In \Cref{subsec:qk_circuit}, we show that the head attends to any token which it is currently predicting.
    \item In \Cref{subsec:how_much_explained}, we define a form of ablation which deletes all mechanisms except for these two, and preserve X\% of our head’s effect on reducing loss. 
\end{enumerate}

\subsection{OV Circuit}
\label{subsec:ov_circuit}

In this section, we present both \textbf{static} and \textbf{dynamic} evidence for how Attention Head 10.7 performs copy suppression. 

\textbf{Static evidence} refers to any evidence that comes from solely weights-based analysis, without running any forward passes (e.g. \citet{elhage2021mathematical} study the eigenvalues of weight matrices). \textbf{Dynamic evidence} refers to any evidence that comes from forward passes (e.g. \citet{wang2023interpretability} perform ablations and use path patching). 

\begin{tcolorbox}[sharp corners, colback=gray!20, colframe=gray!70, title=Effective Embeddings, before title=\vspace{1mm}]

GPT-2 Small uses the same matrix in its embedding and unembedding layers, which may make learning certain tasks harder (for example, \citet{elhage2021mathematical} show that tied embeddings do not allow for bigrams to be modelled perfectly). 

Empirically, several previous works on GPT-2 Small have found that the output of MLP0 is often more important for token predictions than the model’s embedding \citep{wang2023interpretability, greaterthan}, and MLP0 is far more important than any other attention layer or MLP in models trained without dropout \citep{mcgrath2023hydra}.

For this reason, we define the effective embedding matrix $W_{EE} \in \mathbb{R}^{d_{\text{vocab}} \times d_{\text{model}}}$ which has rows for each token $T$ in GPT-2 Small’s vocabulary that are calculated as follows:

\vspace{3mm}

\begin{enumerate}
    \item Take the embedding $W_E$ for the token $T$,
    \item Apply the $0$th attention layer, with all heads' self-attention fixed to one),
    \item Apply the $0$th MLP layer.
\end{enumerate}

\vspace{3mm}

We justify our choice of this matrix in \Cref{app:effective_embedding_analysis}.

\end{tcolorbox}

\subsubsection{Static Evidence}
\label{subsubsec:static_evidence}

In our static experiments, we construct the \textbf{full OV circuit}:\footnote{In this section and the rest of the paper, we use the notation for transformer components from \citet{elhage2021mathematical}.}

$$
W_{EE}W_V W_O W_U
$$

This is defined as the matrix $M$ such that, if $x$ is the one-hot encoded vector of a source token, then the row vector $x^T M$ is the direct logit effect at any sequence position which only attends to $x$. \red{Can't we just say `this is the OV circuit from Elhage et al except with $W_{EE}$"?} If head 10.7 is performing copy suppression, we expect to find that the diagonal elements of this matrix (i.e. the effect on the prediction $x$, when $x$ is attended to) are consistently the most negative elements in their corresponding rows. This is indeed what we find - the median rank of the diagonal element when each row is sorted in ascending order (which we will call the \textbf{self-suppression rank} is 0, indicating that the head is successfully copy-suppressing over half the tokens in the model’s vocabulary. Furthermore, 84.70\% of the vocabulary has a self-suppression rank less than 10.

(TODO - figure)

\begin{tcolorbox}[sharp corners, colback=gray!20, colframe=gray!70, title=Function Words, before title=\vspace{1mm}]

Examining the source tokens for which this head \textit{doesn’t} suppress the prediction proved to be informative. We found a total of 301 words which do not have a self-suppression rank of less than 10\% the size of the total vocabulary. The majority of these (TODO: give number) were \textbf{function words} (e.g. “ a”, “ the”, “ will”, “ some”, “ its”, “ meanwhile”).

\vspace{3mm}

This shows that copy-suppression is not generically used for every token in the vocabulary, rather it is differentially activated depending on the type of word which has been copied. We discuss some possible interpretations and implications of this in the appendix.

\end{tcolorbox}

\subsubsection{Dynamic Evidence}
\label{subsubsec:ov_circuit_dynamic_evidence}
This kind of analysis doesn’t tell us how head 10.7 actually behaves in practice, since the residual stream before layer 10 will have more than just the initial token embedding. To test our hypothesis that 10.7’s OV circuit is mostly copy-suppressing, we performed the following dynamic experiment:

\begin{itemize}
    \item Run a forward pass on a sample of OpenWebText,
    \item Filter for all (source, destination) token pairs where the attention from destination to source is above some threshold (we chose 10\%),
    \item Measure the direct logit attribution of the information moved from each of these source tokens to the corresponding destination token,
    \item Perform the same experiment as we did in the static analysis section (measuring the rank of the source token in this direct logit attribution).
\end{itemize}

We found that the results approximately matched our dynamic analysis (with slightly more noise). The proportion of (source, destination) token pairs where the source token is in the top 10 most suppressed tokens is 78.24\% (which is close to the static analysis result of 84.70\%). 

\begin{tcolorbox}[sharp corners, colback=gray!20, colframe=gray!70, title=Semantic Similarity, before title=\vspace{1mm}]

\red{TODO appendix this}

42.00\% of (source, destination) pairs had the source token in the top 10 most suppressed tokens, but not the most suppressed. When we inspect these cases, we find a common theme: the most suppressed token is often semantically related to the source token. For our purposes, we define \textbf{semantically related} as an equivalence relation on tokens, where  if tokens S and T are related via any of the following:

\begin{itemize}
    \item Capitalization (e.g. “ pier” and “ Pier” are related),
    \item Prepended spaces (e.g. “ token” and “token” are related),
    \item Pluralization (e.g. “ device” and “ devices” are related),
    \item Sharing the same morphological root (e.g. "drive", "driver", "driving" are all related)
    \item Tokenization (e.g. “ Berkeley” and “keley” are related, because the non-space version “Berkeley” is tokenized into [“Ber”, “keley”]).
\end{itemize}

We codify these rules, and find that in 90\% of the aforementioned cases, the most suppressed token is semantically related to the source token. Although part of this is explained by the high cosine similarity between semantically related tokens, this isn't the whole story (on this set of examples, the average cosine similarity between the source token and the semantically related most suppressed token was 0.520). We speculate that the copy suppression algorithm is better thought of as\textbf{ semantic copy suppression}, i.e. all tokens semantically related to the source token are suppressed, rather than \textbf{pure copy suppression} (where only the source token is suppressed). The figure below presents some OpenWebText examples of copy suppression occurring for semantically related tokens.\\

\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{figures/text-figure-2.png}
\captionof{figure}{Examples of semantic similarity.}
\label{fig:semantic_similarity}

\vspace{4mm}

We discuss some implications of this in \Cref{subsec:cspa_mechanism} and Appendix TODO.

\end{tcolorbox}

\subsection{QK Circuit}
\label{subsec:qk_circuit}

In \Cref{subsec:neg_heads_owt} we observed that 10.7 attends to tokens that have been confidently predicted, and in \Cref{subsec:ov_circuit} we showed that 10.7 suppresses predictions when it attends to them. We conjectured that the way that 10.7 attended to confident predictions was by matching a confident prediction in its queryside vector with the (effective) embedding of that token at keyside. This would mean that the attention scores of 10.7 when a token $t$ was predicted queryside and a token $s$ was present in context keyside would be equal to 

\begin{equation}
    \frac{1}{\sqrt{d_{\text{head}}}} W_{EE}[s]^T W_K W_Q^T W_U[t].
\end{equation}

We can then test this theory for a given token $t$ by taking the softmax over all tokens $s$ in a particular context, and looking at the ``attention probability" from token $t$ to itself. We also replace the queryside and keyside lookup tables $W_{EE}$ and $W_U$ with other (un)embeddings to test alternative mechanisms. We computed the average amount that tokens sampled from OpenWebText prompts attended to themselves rather than other tokens in these prompts. Full details of our QK intervention experiments can be found in \Cref{app:qk_intervention_explainer}. The results can be found in \Cref{fig:lookup_tables_self_attention}.

\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=0.68\textwidth]{figures/some_self_attentions.png}
    \caption{How much Attention Head 10.7 causes tokens to attend to themselves when various vectors are used queryside and keyside. \red{TODO move colorbar closer to heatmap}}
    \label{fig:lookup_tables_self_attention}
\end{wrapfigure}

We find that 

\begin{compactenum}
    \item Head 10.7 has greatest token self-attention when the queryside vector is an unembedding vector.
    \item Head 10.7 has greatest token self-attention when the keyside vector involves MLP0.
\end{compactenum}

Head 10.7 has greatest token self-attention when the queryside vector is an unembedding vector, as across all three different keyside embeddings, the token self-attention is maximised when the queryside lookup table is $W_U$. Additionally, the two greatest token self-attention values across all queryside and keyside lookup tables occur when we use either MLP0’s output or the effective embedding, which includes MLP0 (\Cref{subsubsec:static_evidence}). In \Cref{app:lookup_table_self_attention_for_other_heads_in_gpt2_small} we show that in duplicate token heads the greatest token self-attention does not occur when the queryside vector is an unembedding vector, suggesting that 10.7 has a qualitatively different QK-circuit to naive matching.

\subsubsection{Making a more faithful keyside approximation}
\label{subsubsec:more_faithful_keyside}

\red{Arthur is generally underwhelmed by results here - maybe come back to this after sorting out the ablations.}

Is our minimal mechanism for Negative Heads faithful to the computation that occurs on forward passes on dataset examples? To test this, we firstly select some important key tokens which we will measure faithfulness on. We look at the top 5\% of token completions where 10.7 was most useful (as in \Cref{fig:mids_dataset_examples}) and select the top two non-BOS tokens in context that have maximal attention paid to them. We then project 10.7’s key input onto a component parallel to the effective embedding for the key tokens, and calculate the change in attention paid to the selected key tokens.
The resulting distribution of changes in attention can be found in \Cref{fig:effective_embedding_attention_change}.

\begin{figure} % {r}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/effective_embedding_key_change_in_attention.png}
    \caption{Change in attention on tokens when projecting key vectors onto the effective embedding for tokens.}
    \label{fig:effective_embedding_attention_change}
\end{figure}

We find that the median attention change is $-0.09$, with lower quartile $-0.19$. Since the average attention amongst these samples is $0.21$, this suggests that the effective embedding does not faithfully capture the model's attention.

To use a more faithful embedding of keyside tokens, we run a forward pass where we set all attention weights to tokens other than BOS and the current token to 0. We then measure the state of the residual stream before input to Head 10.7, which we call the \textbf{context-free residual state}. Repeating the experiment used to generate \Cref{fig:effective_embedding_attention_change} but using the context-free residual state rather than the effective embedding, we find a more faithful approximation of 10.7's keyside input as \Cref{fig:context_free_residual_attention_change} shows that the change in 10.7’s attention weights is closer to $-0.06$ which is closer to $0$.

\begin{figure} % {r}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/context_free_residual_attention_change.png}
    \caption{Change in attention on tokens when projecting key vectors onto the context free residual state.}
    \label{fig:context_free_residual_attention_change}
\end{figure}

\subsubsection{Making a more faithful queryside approximation}
\label{subsubsec:more_faithful_queryside}

We perform a similar intervention to the components on the input to the model’s query circuit. We study the top 5\% of token completions where 10.7 has most important effect. For the two key tokens with highest attention weight in each of these prompts, we project the query vector onto the unembedding vector for that key token. We then recompute attention probabilities and calculate how much this differs from the unmodified model. We find that again our approximation still causes a lot of attention decrease in many cases (\Cref{fig:query_unembed_projection}).

\begin{figure} % s{r}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/query_unembed_projection.png}
    \caption{Change in attention on tokens when projecting query vectors onto the unembedding vectors for particular tokens.}
    \label{fig:query_unembed_projection}
\end{figure}

There is a component of the queryside input perpendicular to the unembedding direction that is important for 10.7’s attention. This component seems more important for 10.7s attention when the unembedding direction is more important, by performing an identical experiment to the experiment that produced \Cref{fig:query_unembed_projection} except projecting onto the perpendicular direction, and then measuring the correlation between the attention change for both of these interventions on each prompt, shown in \Cref{fig:query_unembed_perp_correlation}. \red{Highlight that this is direct effect only}

\begin{figure} % {r}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/query_unembed_perp_correlation.png}
    \caption{Correlation between change in attention on tokens when projecting onto the component parallel to the unembedding and ($x$-axis) and also projecting onto the component perpendicular to the unembedding ($y$-axis). \red{TODO it's plausible that this correlation is obvious, because it keeps key bias or something. Arthur check. Also bigger text}}
    \label{fig:query_unembed_perp_correlation}
\end{figure}

We’re not sure what this perpendicular component represents. \Cref{subsec:self_repair_component_intervention_complication} dives deeper into  this perpendicular component in the IOI case study, where we show further that the components that output large unembedding vectors (the Name Mover heads) also output large perpendicular components, too. 

\subsection{How much of 10.7's behavior have we explained?}
\label{subsec:how_much_explained}

In this section, we define a form of ablation which deletes all information moved from source to destination tokens *except for* the information which comes directly from the copy suppression mechanism. We will refer to this as **Copy Suppression-Preserving Ablation (CSPA)**. First, we explain exactly how this ablation works. Then we present the result of this ablation, showing that it is much closer to performing no ablation than to a full ablation (indicating that we have correctly identified the critical channel which the head uses to effect loss).

\subsubsection{CSPA Mechanism}
\label{subsec:cspa_mechanism}

The core mechanism of copy suppression can be described as follows:

\begin{adjustwidth}{5mm}{5mm}\red{Are we going to include semantically similar ablations in the main text? (No)} At destination token $d$, token $s^*$ is predicted. This token is semantically related to some token $s$ which appears earlier in context. This causes us to attend back to token $s$, and the resulting attention vector suppresses the prediction of $s^*$.\end{adjustwidth}

Based on this, we choose the following ablation method depending on the hyperparameter $K$:

\begin{adjustwidth}{5mm}{5mm}\red{TODO: make consistent with the Section 3.2 where we used destination $D$ and source $S$ not lower case.} For each destination token $d$, find all tokens $s^*$ which are semantically similar to tokens that appear in context before $d$, and choose the subset of $K$ which are currently predicted with highest probability. This gives us a set of $K$ pairs $(s, s^*)$. For each source token $s$, we project the corresponding result vector onto the span of the set of unembeddings of all semantically related tokens $s^*$ where $s^*$ is in one of the $K$ pairs $(s, s^*)$.\end{adjustwidth}

As an example of how this might work, consider the ``America's private prisons'' prompt from \Cref{fig:semantic_similarity}. In this case the destination token $d$ is `` private". The predicted token $s^*$ is `` prison", which is semantically related to the `` prisons" which appears earlier in context and so is the source token $s$. So we would project the result vector from the source token `` prisons" onto the unembedding for the token `` prison".

% TODO integrate into first paragraphs of 4.3:
% \item We are measuring the direct effect of this head, rather than the effect through other components in the model, since (as we have discussed earlier in this paper) we believe that the majority of the effect of this head is direct.

This ablation is actually stricter than copy-suppression, because it also tests the hypothesis of \textbf{sparsity} - that in normal operation, the majority of the head's effect comes from just one source token.

\subsubsection{Results of CSPA}

(TODO)

\begin{figure} % s{r}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/ablation-diagrams.png}
    \caption{Diagram of the different versions of head ablation we use.}
    \label{fig:ablation_diagrams}
\end{figure}

\newpage
